Tiled QR factorization algorithms

This work revisits existing algorithms for the QR factorization of rectangular matrices composed of p-by-q tiles, where p >= q. Within this framework, we study the critical paths and performance of algorithms such as Sameh and Kuck, Modi and Clarke, Greedy, and those found within PLASMA. Although neither Modi and Clarke nor Greedy is optimal, both are shown to be asymptotically optimal for all matrices of size p = q^2 f(q), where f is any function such that \lim_{+\infty} f= 0. This novel and important complexity result applies to all matrices where p and q are proportional, p = \lambda q, with \lambda >= 1, thereby encompassing many important situations in practice (least squares). We provide an extensive set of experiments that show the superiority of the new algorithms for tall matrices.

==> fig/perf_factorization_kernels_d.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\TSQRT (in)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\GEQRT (in)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\TTQRT (in)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\GEQRT+\TTQRT (in)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\GEMM (in)\\\textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\TSQRT (out)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\GEQRT (out)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\TTQRT (out)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\GEQRT+\TTQRT (out)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\GEMM (out) \end{tabular}}}%
\psfrag{018}[bc][bc]{\matlabtextA GFLOP/s}%
\psfrag{019}[tc][tc]{\matlabtextA tile size}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $100$}%
\psfrag{001}[ct][ct]{\matlabtextA $200$}%
\psfrag{002}[ct][ct]{\matlabtextA $300$}%
\psfrag{003}[ct][ct]{\matlabtextA $400$}%
\psfrag{004}[ct][ct]{\matlabtextA $500$}%
\psfrag{005}[ct][ct]{\matlabtextA $600$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $1$}%
\psfrag{008}[rc][rc]{\matlabtextA $2$}%
\psfrag{009}[rc][rc]{\matlabtextA $3$}%
\psfrag{010}[rc][rc]{\matlabtextA $4$}%
\psfrag{011}[rc][rc]{\matlabtextA $5$}%
\psfrag{012}[rc][rc]{\matlabtextA $6$}%
\psfrag{013}[rc][rc]{\matlabtextA $7$}%
\psfrag{014}[rc][rc]{\matlabtextA $8$}%
\psfrag{015}[rc][rc]{\matlabtextA $9$}%
\psfrag{016}[rc][rc]{\matlabtextA $10$}%
%
%% </ytick>

==> fig/perf_factorization_kernels_z.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\TSQRT (in)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\GEQRT (in)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\TTQRT (in)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\GEQRT+\TTQRT (in)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\GEMM (in)\\\textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\TSQRT (out)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\GEQRT (out)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\TTQRT (out)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\GEQRT+\TTQRT (out)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\GEMM (out) \end{tabular}}}%
\psfrag{018}[bc][bc]{\matlabtextA GFLOP/s}%
\psfrag{019}[tc][tc]{\matlabtextA tile size}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $100$}%
\psfrag{001}[ct][ct]{\matlabtextA $200$}%
\psfrag{002}[ct][ct]{\matlabtextA $300$}%
\psfrag{003}[ct][ct]{\matlabtextA $400$}%
\psfrag{004}[ct][ct]{\matlabtextA $500$}%
\psfrag{005}[ct][ct]{\matlabtextA $600$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $1$}%
\psfrag{008}[rc][rc]{\matlabtextA $2$}%
\psfrag{009}[rc][rc]{\matlabtextA $3$}%
\psfrag{010}[rc][rc]{\matlabtextA $4$}%
\psfrag{011}[rc][rc]{\matlabtextA $5$}%
\psfrag{012}[rc][rc]{\matlabtextA $6$}%
\psfrag{013}[rc][rc]{\matlabtextA $7$}%
\psfrag{014}[rc][rc]{\matlabtextA $8$}%
\psfrag{015}[rc][rc]{\matlabtextA $9$}%
\psfrag{016}[rc][rc]{\matlabtextA $10$}%
%
%% </ytick>

==> fig/perf_update_kernels_d.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\TSMQR (in)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\ORMQR (in)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\TTMQR (in)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\ORMQR+\TTMQR (in)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\GEMM (in)\\\textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\TSMQR (out)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\ORMQR (out)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\TTMQR (out)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\ORMQR+\TTMQR (out)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\GEMM (out) \end{tabular}}}%
\psfrag{018}[bc][bc]{\matlabtextA GFLOP/s}%
\psfrag{019}[tc][tc]{\matlabtextA tile size}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $100$}%
\psfrag{001}[ct][ct]{\matlabtextA $200$}%
\psfrag{002}[ct][ct]{\matlabtextA $300$}%
\psfrag{003}[ct][ct]{\matlabtextA $400$}%
\psfrag{004}[ct][ct]{\matlabtextA $500$}%
\psfrag{005}[ct][ct]{\matlabtextA $600$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $1$}%
\psfrag{008}[rc][rc]{\matlabtextA $2$}%
\psfrag{009}[rc][rc]{\matlabtextA $3$}%
\psfrag{010}[rc][rc]{\matlabtextA $4$}%
\psfrag{011}[rc][rc]{\matlabtextA $5$}%
\psfrag{012}[rc][rc]{\matlabtextA $6$}%
\psfrag{013}[rc][rc]{\matlabtextA $7$}%
\psfrag{014}[rc][rc]{\matlabtextA $8$}%
\psfrag{015}[rc][rc]{\matlabtextA $9$}%
\psfrag{016}[rc][rc]{\matlabtextA $10$}%
%
%% </ytick>

==> fig/perf_update_kernels_z.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\TSMQR (in)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\UNMQR (in)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\TTMQR (in)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\UNMQR+\TTMQR (in)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}\hspace{0.55em}\rule[0.5ex]{0.625em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\GEMM (in)\\\textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\TSMQR (out)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\UNMQR (out)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\TTMQR (out)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\UNMQR+\TTMQR (out)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\GEMM (out) \end{tabular}}}%
\psfrag{018}[bc][bc]{\matlabtextA GFLOP/s}%
\psfrag{019}[tc][tc]{\matlabtextA tile size}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $100$}%
\psfrag{001}[ct][ct]{\matlabtextA $200$}%
\psfrag{002}[ct][ct]{\matlabtextA $300$}%
\psfrag{003}[ct][ct]{\matlabtextA $400$}%
\psfrag{004}[ct][ct]{\matlabtextA $500$}%
\psfrag{005}[ct][ct]{\matlabtextA $600$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $1$}%
\psfrag{008}[rc][rc]{\matlabtextA $2$}%
\psfrag{009}[rc][rc]{\matlabtextA $3$}%
\psfrag{010}[rc][rc]{\matlabtextA $4$}%
\psfrag{011}[rc][rc]{\matlabtextA $5$}%
\psfrag{012}[rc][rc]{\matlabtextA $6$}%
\psfrag{013}[rc][rc]{\matlabtextA $7$}%
\psfrag{014}[rc][rc]{\matlabtextA $8$}%
\psfrag{015}[rc][rc]{\matlabtextA $9$}%
\psfrag{016}[rc][rc]{\matlabtextA $10$}%
%
%% </ytick>

==> fig/results_AA_p40_IG_d_48_8000_pic1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{020}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [1   3   6  11  12  18  32]\\Best domain size for \PT (TT) = [1   3  10   5  17  27  19]\end{tabular}}%
\psfrag{021}[bc][bc]{\matlabtextA GFLOP/s}%
\psfrag{022}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $0$}%
\psfrag{014}[rc][rc]{\matlabtextA $50$}%
\psfrag{015}[rc][rc]{\matlabtextA $100$}%
\psfrag{016}[rc][rc]{\matlabtextA $150$}%
\psfrag{017}[rc][rc]{\matlabtextA $200$}%
\psfrag{018}[rc][rc]{\matlabtextA $250$}%
%
%% </ytick>

==> fig/results_AA_p40_IG_d_48_8000_pic2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{022}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [1   3   6  11  12  18  32]\\Best domain size for \PT (TT) = [1   3  10   5  17  27  19]\end{tabular}}%
\psfrag{023}[bc][bc]{\matlabtextA Overhead in time with respect to \Greedy (\Greedy = 1)}%
\psfrag{024}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $1$}%
\psfrag{014}[rc][rc]{\matlabtextA $2$}%
\psfrag{015}[rc][rc]{\matlabtextA $3$}%
\psfrag{016}[rc][rc]{\matlabtextA $4$}%
\psfrag{017}[rc][rc]{\matlabtextA $5$}%
\psfrag{018}[rc][rc]{\matlabtextA $6$}%
\psfrag{019}[rc][rc]{\matlabtextA $7$}%
\psfrag{020}[rc][rc]{\matlabtextA $8$}%
%
%% </ytick>

==> fig/results_AA_p40_IG_d_48_8000_pic3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{022}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [1   3   6  11  12  18  32]\\Best domain size for \PT (TT) = [1   3  10   5  17  27  19]\end{tabular}}%
\psfrag{023}[bc][bc]{\matlabtextA Overhead in time with respect to \Greedy (\Greedy = 1)}%
\psfrag{024}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{014}[rc][rc]{\matlabtextA $0.9$}%
\psfrag{015}[rc][rc]{\matlabtextA $1$}%
\psfrag{016}[rc][rc]{\matlabtextA $1.1$}%
\psfrag{017}[rc][rc]{\matlabtextA $1.2$}%
\psfrag{018}[rc][rc]{\matlabtextA $1.3$}%
\psfrag{019}[rc][rc]{\matlabtextA $1.4$}%
\psfrag{020}[rc][rc]{\matlabtextA $1.5$}%
%
%% </ytick>

==> fig/results_AA_p40_IG_z_48_8000_pic1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{023}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [1   3   5  10  11   8   4]\\Best domain size for \PT (TT) = [1   5   5   5  17  28   8]\end{tabular}}%
\psfrag{024}[bc][bc]{\matlabtextA GFLOP/s}%
\psfrag{025}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $0$}%
\psfrag{014}[rc][rc]{\matlabtextA $20$}%
\psfrag{015}[rc][rc]{\matlabtextA $40$}%
\psfrag{016}[rc][rc]{\matlabtextA $60$}%
\psfrag{017}[rc][rc]{\matlabtextA $80$}%
\psfrag{018}[rc][rc]{\matlabtextA $100$}%
\psfrag{019}[rc][rc]{\matlabtextA $120$}%
\psfrag{020}[rc][rc]{\matlabtextA $140$}%
\psfrag{021}[rc][rc]{\matlabtextA $160$}%
%
%% </ytick>

==> fig/results_AA_p40_IG_z_48_8000_pic2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{024}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [1   3   5  10  11   8   4]\\Best domain size for \PT (TT) = [1   5   5   5  17  28   8]\end{tabular}}%
\psfrag{025}[bc][bc]{\matlabtextA Overhead in time with respect to \Greedy (\Greedy = 1)}%
\psfrag{026}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $1$}%
\psfrag{014}[rc][rc]{\matlabtextA $2$}%
\psfrag{015}[rc][rc]{\matlabtextA $3$}%
\psfrag{016}[rc][rc]{\matlabtextA $4$}%
\psfrag{017}[rc][rc]{\matlabtextA $5$}%
\psfrag{018}[rc][rc]{\matlabtextA $6$}%
\psfrag{019}[rc][rc]{\matlabtextA $7$}%
\psfrag{020}[rc][rc]{\matlabtextA $8$}%
\psfrag{021}[rc][rc]{\matlabtextA $9$}%
\psfrag{022}[rc][rc]{\matlabtextA $10$}%
%
%% </ytick>

==> fig/results_AA_p40_IG_z_48_8000_pic3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{025}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [1   3   5  10  11   8   4]\\Best domain size for \PT (TT) = [1   5   5   5  17  28   8]\end{tabular}}%
\psfrag{026}[bc][bc]{\matlabtextA Overhead in time with respect to \Greedy (\Greedy = 1)}%
\psfrag{027}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $0.95$}%
\psfrag{014}[rc][rc]{\matlabtextA $1$}%
\psfrag{015}[rc][rc]{\matlabtextA $1.05$}%
\psfrag{016}[rc][rc]{\matlabtextA $1.1$}%
\psfrag{017}[rc][rc]{\matlabtextA $1.15$}%
\psfrag{018}[rc][rc]{\matlabtextA $1.2$}%
\psfrag{019}[rc][rc]{\matlabtextA $1.25$}%
\psfrag{020}[rc][rc]{\matlabtextA $1.3$}%
\psfrag{021}[rc][rc]{\matlabtextA $1.35$}%
\psfrag{022}[rc][rc]{\matlabtextA $1.4$}%
\psfrag{023}[rc][rc]{\matlabtextA $1.45$}%
%
%% </ytick>

==> fig/results_AA_p40_pic1_d.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{019}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [ 1 1 1 1 5 5 5 5 5 5 10 ... 10 ]\\Best domain size for \PT (TT) = [ 1 3 5 5 5 10 10 10 10 10 20 ... 20 ]\end{tabular}}%
\psfrag{020}[bc][bc]{\matlabtextA Predicted GFLOP/s}%
\psfrag{021}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $50$}%
\psfrag{014}[rc][rc]{\matlabtextA $100$}%
\psfrag{015}[rc][rc]{\matlabtextA $150$}%
\psfrag{016}[rc][rc]{\matlabtextA $200$}%
\psfrag{017}[rc][rc]{\matlabtextA $250$}%
%
%% </ytick>

==> fig/results_AA_p40_pic1_z.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{022}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [ 1 1 1 1 5 5 5 5 5 5 10 ... 10 ]\\Best domain size for \PT (TT) = [ 1 3 5 5 5 10 10 10 10 10 20 ... 20 ]\end{tabular}}%
\psfrag{023}[bc][bc]{\matlabtextA Predicted GFLOP/s}%
\psfrag{024}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $20$}%
\psfrag{014}[rc][rc]{\matlabtextA $40$}%
\psfrag{015}[rc][rc]{\matlabtextA $60$}%
\psfrag{016}[rc][rc]{\matlabtextA $80$}%
\psfrag{017}[rc][rc]{\matlabtextA $100$}%
\psfrag{018}[rc][rc]{\matlabtextA $120$}%
\psfrag{019}[rc][rc]{\matlabtextA $140$}%
\psfrag{020}[rc][rc]{\matlabtextA $160$}%
%
%% </ytick>

==> fig/results_AA_p40_pic2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{024}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [ 1 1 1 1 5 5 5 5 5 5 10 ... 10 ]\\Best domain size for \PT (TT) = [ 1 3 5 5 5 10 10 10 10 10 20 ... 20 ]\end{tabular}}%
\psfrag{025}[bc][bc]{\matlabtextA Overhead in cp length with respect to \Greedy (\Greedy = 1)}%
\psfrag{026}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $1$}%
\psfrag{014}[rc][rc]{\matlabtextA $2$}%
\psfrag{015}[rc][rc]{\matlabtextA $3$}%
\psfrag{016}[rc][rc]{\matlabtextA $4$}%
\psfrag{017}[rc][rc]{\matlabtextA $5$}%
\psfrag{018}[rc][rc]{\matlabtextA $6$}%
\psfrag{019}[rc][rc]{\matlabtextA $7$}%
\psfrag{020}[rc][rc]{\matlabtextA $8$}%
\psfrag{021}[rc][rc]{\matlabtextA $9$}%
\psfrag{022}[rc][rc]{\matlabtextA $10$}%
%
%% </ytick>

==> fig/results_AA_p40_pic3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{025}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [ 1 1 1 1 5 5 5 5 5 5 10 ... 10 ]\\Best domain size for \PT (TT) = [ 1 3 5 5 5 10 10 10 10 10 20 ... 20 ]\end{tabular}}%
\psfrag{026}[bc][bc]{\matlabtextA Overhead in cp length with respect to \Greedy (\Greedy = 1)}%
\psfrag{027}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $0.95$}%
\psfrag{014}[rc][rc]{\matlabtextA $1$}%
\psfrag{015}[rc][rc]{\matlabtextA $1.05$}%
\psfrag{016}[rc][rc]{\matlabtextA $1.1$}%
\psfrag{017}[rc][rc]{\matlabtextA $1.15$}%
\psfrag{018}[rc][rc]{\matlabtextA $1.2$}%
\psfrag{019}[rc][rc]{\matlabtextA $1.25$}%
\psfrag{020}[rc][rc]{\matlabtextA $1.3$}%
\psfrag{021}[rc][rc]{\matlabtextA $1.35$}%
\psfrag{022}[rc][rc]{\matlabtextA $1.4$}%
\psfrag{023}[rc][rc]{\matlabtextA $1.45$}%
%
%% </ytick>

==> fig/results_AA_p40_pic4.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{1,0.64706,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{1,0.64706,0}{}} & \hspace{0.5em}\FT (TS)\\\textcolor[rgb]{0,0.6,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0,0.6,0}{}} & \hspace{0.5em}\PT (TS) (best)\\\textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{021}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}Best domain size for \PT (TS) = [ 1 1 1 1 5 5 5 5 5 5 10 ... 10 ]\\Best domain size for \PT (TT) = [ 1 3 5 5 5 10 10 10 10 10 20 ... 20 ]\end{tabular}}%
\psfrag{022}[bc][bc]{\matlabtextA Critical path length}%
\psfrag{023}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $200$}%
\psfrag{014}[rc][rc]{\matlabtextA $400$}%
\psfrag{015}[rc][rc]{\matlabtextA $600$}%
\psfrag{016}[rc][rc]{\matlabtextA $800$}%
\psfrag{017}[rc][rc]{\matlabtextA $1000$}%
\psfrag{018}[rc][rc]{\matlabtextA $1200$}%
\psfrag{019}[rc][rc]{\matlabtextA $1400$}%
%
%% </ytick>

==> fig/results_TT_p40_IG_d_48_8000_pic1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{024}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [1   3  10   5  17  27  19]}%
\psfrag{025}[bc][bc]{\matlabtextA GFLOP/s}%
\psfrag{026}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $0$}%
\psfrag{014}[rc][rc]{\matlabtextA $20$}%
\psfrag{015}[rc][rc]{\matlabtextA $40$}%
\psfrag{016}[rc][rc]{\matlabtextA $60$}%
\psfrag{017}[rc][rc]{\matlabtextA $80$}%
\psfrag{018}[rc][rc]{\matlabtextA $100$}%
\psfrag{019}[rc][rc]{\matlabtextA $120$}%
\psfrag{020}[rc][rc]{\matlabtextA $140$}%
\psfrag{021}[rc][rc]{\matlabtextA $160$}%
\psfrag{022}[rc][rc]{\matlabtextA $180$}%
%
%% </ytick>

==> fig/results_TT_p40_IG_d_48_8000_pic2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{023}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [1   3  10   5  17  27  19]}%
\psfrag{024}[bc][bc]{\matlabtextA Overhead in time with respect to \Greedy (\Greedy = 1)}%
\psfrag{025}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $1$}%
\psfrag{014}[rc][rc]{\matlabtextA $1.5$}%
\psfrag{015}[rc][rc]{\matlabtextA $2$}%
\psfrag{016}[rc][rc]{\matlabtextA $2.5$}%
\psfrag{017}[rc][rc]{\matlabtextA $3$}%
\psfrag{018}[rc][rc]{\matlabtextA $3.5$}%
\psfrag{019}[rc][rc]{\matlabtextA $4$}%
\psfrag{020}[rc][rc]{\matlabtextA $4.5$}%
\psfrag{021}[rc][rc]{\matlabtextA $5$}%
%
%% </ytick>

==> fig/results_TT_p40_IG_d_48_8000_pic3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{025}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [1   3  10   5  17  27  19]}%
\psfrag{026}[bc][bc]{\matlabtextA Overhead in time with respect to \Greedy (\Greedy = 1)}%
\psfrag{027}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $0.95$}%
\psfrag{014}[rc][rc]{\matlabtextA $1$}%
\psfrag{015}[rc][rc]{\matlabtextA $1.05$}%
\psfrag{016}[rc][rc]{\matlabtextA $1.1$}%
\psfrag{017}[rc][rc]{\matlabtextA $1.15$}%
\psfrag{018}[rc][rc]{\matlabtextA $1.2$}%
\psfrag{019}[rc][rc]{\matlabtextA $1.25$}%
\psfrag{020}[rc][rc]{\matlabtextA $1.3$}%
\psfrag{021}[rc][rc]{\matlabtextA $1.35$}%
\psfrag{022}[rc][rc]{\matlabtextA $1.4$}%
\psfrag{023}[rc][rc]{\matlabtextA $1.45$}%
%
%% </ytick>

==> fig/results_TT_p40_IG_z_48_8000_pic1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{023}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [1   5   5   5  17  28   8]}%
\psfrag{024}[bc][bc]{\matlabtextA GFLOP/s}%
\psfrag{025}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $0$}%
\psfrag{014}[rc][rc]{\matlabtextA $20$}%
\psfrag{015}[rc][rc]{\matlabtextA $40$}%
\psfrag{016}[rc][rc]{\matlabtextA $60$}%
\psfrag{017}[rc][rc]{\matlabtextA $80$}%
\psfrag{018}[rc][rc]{\matlabtextA $100$}%
\psfrag{019}[rc][rc]{\matlabtextA $120$}%
\psfrag{020}[rc][rc]{\matlabtextA $140$}%
\psfrag{021}[rc][rc]{\matlabtextA $160$}%
%
%% </ytick>

==> fig/results_TT_p40_IG_z_48_8000_pic2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{023}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [1   5   5   5  17  28   8]}%
\psfrag{024}[bc][bc]{\matlabtextA Overhead in time with respect to \Greedy (\Greedy = 1)}%
\psfrag{025}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $1$}%
\psfrag{014}[rc][rc]{\matlabtextA $1.5$}%
\psfrag{015}[rc][rc]{\matlabtextA $2$}%
\psfrag{016}[rc][rc]{\matlabtextA $2.5$}%
\psfrag{017}[rc][rc]{\matlabtextA $3$}%
\psfrag{018}[rc][rc]{\matlabtextA $3.5$}%
\psfrag{019}[rc][rc]{\matlabtextA $4$}%
\psfrag{020}[rc][rc]{\matlabtextA $4.5$}%
\psfrag{021}[rc][rc]{\matlabtextA $5$}%
%
%% </ytick>

==> fig/results_TT_p40_IG_z_48_8000_pic3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{025}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [1   5   5   5  17  28   8]}%
\psfrag{026}[bc][bc]{\matlabtextA Overhead in time with respect to \Greedy (\Greedy = 1)}%
\psfrag{027}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $0.95$}%
\psfrag{014}[rc][rc]{\matlabtextA $1$}%
\psfrag{015}[rc][rc]{\matlabtextA $1.05$}%
\psfrag{016}[rc][rc]{\matlabtextA $1.1$}%
\psfrag{017}[rc][rc]{\matlabtextA $1.15$}%
\psfrag{018}[rc][rc]{\matlabtextA $1.2$}%
\psfrag{019}[rc][rc]{\matlabtextA $1.25$}%
\psfrag{020}[rc][rc]{\matlabtextA $1.3$}%
\psfrag{021}[rc][rc]{\matlabtextA $1.35$}%
\psfrag{022}[rc][rc]{\matlabtextA $1.4$}%
\psfrag{023}[rc][rc]{\matlabtextA $1.45$}%
%
%% </ytick>

==> fig/results_TT_p40_pic1_d.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{023}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [ 1 3 5 5 5 10 10 10 10 10 20 \ldots 20 ]}%
\psfrag{024}[bc][bc]{\matlabtextA Predicted GFLOP/s}%
\psfrag{025}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $20$}%
\psfrag{014}[rc][rc]{\matlabtextA $40$}%
\psfrag{015}[rc][rc]{\matlabtextA $60$}%
\psfrag{016}[rc][rc]{\matlabtextA $80$}%
\psfrag{017}[rc][rc]{\matlabtextA $100$}%
\psfrag{018}[rc][rc]{\matlabtextA $120$}%
\psfrag{019}[rc][rc]{\matlabtextA $140$}%
\psfrag{020}[rc][rc]{\matlabtextA $160$}%
\psfrag{021}[rc][rc]{\matlabtextA $180$}%
%
%% </ytick>

==> fig/results_TT_p40_pic1_z.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[br][br]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{022}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [ 1 3 5 5 5 10 10 10 10 10 20 \ldots 20 ]}%
\psfrag{023}[bc][bc]{\matlabtextA Predicted GFLOP/s}%
\psfrag{024}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $20$}%
\psfrag{014}[rc][rc]{\matlabtextA $40$}%
\psfrag{015}[rc][rc]{\matlabtextA $60$}%
\psfrag{016}[rc][rc]{\matlabtextA $80$}%
\psfrag{017}[rc][rc]{\matlabtextA $100$}%
\psfrag{018}[rc][rc]{\matlabtextA $120$}%
\psfrag{019}[rc][rc]{\matlabtextA $140$}%
\psfrag{020}[rc][rc]{\matlabtextA $160$}%
%
%% </ytick>

==> fig/results_TT_p40_pic2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{023}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [ 1 3 5 5 5 10 10 10 10 10 20 \ldots 20 ]}%
\psfrag{024}[bc][bc]{\matlabtextA Overhead in cp length with respect to \Greedy (\Greedy = 1)}%
\psfrag{025}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $1$}%
\psfrag{014}[rc][rc]{\matlabtextA $1.5$}%
\psfrag{015}[rc][rc]{\matlabtextA $2$}%
\psfrag{016}[rc][rc]{\matlabtextA $2.5$}%
\psfrag{017}[rc][rc]{\matlabtextA $3$}%
\psfrag{018}[rc][rc]{\matlabtextA $3.5$}%
\psfrag{019}[rc][rc]{\matlabtextA $4$}%
\psfrag{020}[rc][rc]{\matlabtextA $4.5$}%
\psfrag{021}[rc][rc]{\matlabtextA $5$}%
%
%% </ytick>

==> fig/results_TT_p40_pic3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[tr][tr]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{025}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [ 1 3 5 5 5 10 10 10 10 10 20 \ldots 20 ]}%
\psfrag{026}[bc][bc]{\matlabtextA Overhead in cp length with respect to \Greedy (\Greedy = 1)}%
\psfrag{027}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $0.95$}%
\psfrag{014}[rc][rc]{\matlabtextA $1$}%
\psfrag{015}[rc][rc]{\matlabtextA $1.05$}%
\psfrag{016}[rc][rc]{\matlabtextA $1.1$}%
\psfrag{017}[rc][rc]{\matlabtextA $1.15$}%
\psfrag{018}[rc][rc]{\matlabtextA $1.2$}%
\psfrag{019}[rc][rc]{\matlabtextA $1.25$}%
\psfrag{020}[rc][rc]{\matlabtextA $1.3$}%
\psfrag{021}[rc][rc]{\matlabtextA $1.35$}%
\psfrag{022}[rc][rc]{\matlabtextA $1.4$}%
\psfrag{023}[rc][rc]{\matlabtextA $1.45$}%
%
%% </ytick>

==> fig/results_TT_p40_pic4.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[tl][tl]{\matlabtextA \setlength{\fboxsep}{5pt}\setlength{\fboxrule}{0.5pt}\fcolorbox{black}{white}{\begin{tabular}{cl} \textcolor[rgb]{0.57647,0,0}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.57647,0,0}{}} & \hspace{0.5em}\FT (TT)\\\textcolor[rgb]{0.54118,0.16863,0.88627}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.54118,0.16863,0.88627}{}} & \hspace{0.5em}\PT (TT) (best)\\\textcolor[rgb]{0.46667,0.53333,0.6}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.46667,0.53333,0.6}{}} & \hspace{0.5em}\MC (TT)\\\textcolor[rgb]{0.2549,0.41176,0.88235}{\rule[0.5ex]{3em}{2pt}} \put(-19,1){\textcolor[rgb]{0,0,0}{}}  \put(-19,1){\textcolor[rgb]{0.2549,0.41176,0.88235}{}} & \hspace{0.5em}\Greedy \end{tabular}}}%
\psfrag{021}[bc][bc]{\matlabtextA Best domain size for \PT (TT) = [ 1 3 5 5 5 10 10 10 10 10 20 \ldots 20 ]}%
\psfrag{022}[bc][bc]{\matlabtextA Critical path length}%
\psfrag{023}[tc][tc]{\matlabtextA $q$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $3$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $5$}%
\psfrag{005}[ct][ct]{\matlabtextA $6$}%
\psfrag{006}[ct][ct]{\matlabtextA $7$}%
\psfrag{007}[ct][ct]{\matlabtextA $8$}%
\psfrag{008}[ct][ct]{\matlabtextA $9$}%
\psfrag{009}[ct][ct]{\matlabtextA $10$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
\psfrag{011}[ct][ct]{\matlabtextA $30$}%
\psfrag{012}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextA $200$}%
\psfrag{014}[rc][rc]{\matlabtextA $400$}%
\psfrag{015}[rc][rc]{\matlabtextA $600$}%
\psfrag{016}[rc][rc]{\matlabtextA $800$}%
\psfrag{017}[rc][rc]{\matlabtextA $1000$}%
\psfrag{018}[rc][rc]{\matlabtextA $1200$}%
\psfrag{019}[rc][rc]{\matlabtextA $1400$}%
%
%% </ytick>
